Video Question Generation via Cross-Modal Self-Attention Networks Learning

We introduce a novel task, Video Question Generation (Video QG). A Video QG model automatically generates questions given a video clip and its corresponding dialogues. Video QG requires a range of skills -- sentence comprehension, temporal relation, the interplay between vision and language, and the ability to ask meaningful questions. To address this, we propose a novel semantic rich cross-modal self-attention (SRCMSA) network to aggregate the multi-modal and diverse features. To be more precise, we enhance the video frames semantic by integrating the object-level information, and we jointly consider the cross-modal attention for the video question generation task. Excitingly, our proposed model remarkably improves the baseline from 7.58 to 14.48 in the BLEU-4 score on the TVQA dataset. Most of all, we arguably pave a novel path toward understanding the challenging video input and we provide detailed analysis in terms of diversity, which ushers the avenues for future investigations.

==> figure/QoQ.tex <==
\begin{figure*}
  \includegraphics[width=\textwidth]{figure/mmunans1_small.pdf}
  \caption{Generated Unanswerable Questions. Left block: Action Error. The action ``laying on the bed" does not occurs in the clip, making the question unanswerable. Right block: Entity Error. The entity ``patient" is not in the dialogue. cf. section \ref{section:err} }
  \label{fig:unans}
\end{figure*}

\begin{figure*}
  \includegraphics[width=\textwidth]{figure/mmbad_small.pdf}
  \caption{Some answerable but suboptimal questions. Left block: Redundant relation Error. The temporal relation information ``when he say I don't" is unnecessary for ``wearing" because the person do not change the clothes. Right block: General Question. The question can be applied to any video clip with people talking, which is very common in the data.cf. section \ref{section:err}}
  \label{fig:bad}
\end{figure*}

==> figure/back.tex <==
\iffalse
\begin{figure*}
  \includegraphics[width=\textwidth]{figure/cherries.pdf}
  \caption{
  Generated Questions. V: Video, S: Subtitles, GT: Ground Truth, QT (w/o Sub): The question generated with video only. Q (w/sub): The question generated with both video and subtitles. Our proposed model generates more diverse and specific question according to the video and subtitles (\textcolor{red}{red}) while the \baseline{} and \multibaseline{} generate more general ones. [Best viewed in color]}
  \label{fig:cherries}
\end{figure*}
\begin{figure*}
  \includegraphics[width=\textwidth]{figure/mmunans1_small.pdf}
  \caption{Generated Unanswerable Questions. Left block: Action Error. The action ``laying on the bed" does not occurs in the clip, making the question unanswerable. Right block: Entity Error. The entity ``patient" is not in the dialogue. cf. section \ref{section:err} }
  \label{fig:unans}
\end{figure*}

\begin{figure*}
  \includegraphics[width=\textwidth]{figure/mmbad_small.pdf}
  \caption{Some answerable but suboptimal questions. Left block: Redundant relation Error. The temporal relation information ``when he say I don't" is unnecessary for ``wearing" because the person do not change the clothes. Right block: General Question. The question can be applied to any video clip with people talking, which is very common in the data.cf. section \ref{section:err}}
  \label{fig:bad}
\end{figure*}

\fi

\iffalse
\subsection{Vanilla Transformer Encoder}
In this section, we first introduce the vanilla transformer \cite{transformer} which inspires our SRCMSA network.
\newline
\textbf{Scaled Dot-Product Attention}.
%\subsubsection{Scaled Dot-Product Attention}
We start the transformer by explaining the scale dot-product attention, which is the main computation of the transformer. Given a query ${q}_{{t}^{'}}{\in{\mathbb{R}}^{d}}$, where ${t}^{'}$ is the time step of a ${T}^{'}$ queries sequence, a set of keys ${k}_{t}{\in{\mathbb{R}}^{d}}$ and a set of values ${v}_{t}{\in{\mathbb{R}}^{d}}$ from all $T$ keys and values, we compute the dot products of the query with all keys, divide each by $\sqrt{d}$, and apply the softmax function to obtain the weights on the values. In practice, we pack ${q}_{{t}^{'}}$, ${k}_{t}$, and ${v}_{t}$ into matrices $Q$, $K$, and $V$ to compute the attention scores simultaneously. The attention matrix is computed as:
\begin{equation}
Attention(Q, K, V) = softmax(\frac{QK}{\sqrt{d}})V 
\end{equation}
In our experiment, we set K, V as the two different projected subtitles and Q is fed with self-attention SRE.
\newline
\textbf{Multi-Head Attention}.
%\subsubsection{Multi-Head Attention}
A single attention matrix computation is called a ``head", and we adopt the \textit{mutli-head attention} in our model. The multi-head attention consists of \textit{H} parallel heads which allow the model to jointly learn from different representation subspaces. The multi-head attention output is computed as below:
\begin{align}\label{eq:multihead}
& {head}_{j} = Attention({W}_{j}^{Q}Q, {W}_{j}^{K}K, {W}_{j}^{V}V) \\
 & MultiHead(Q, K, V) = {W}^{O}Concat({head}_{1},...,{head}_{H}) 
\end{align}

where ${W}_{j}^{Q}$, ${W}_{j}^{K}$, and ${W}_{j}^{V} \in{{\mathbb{R}}^{\frac{d}{H} \times d}}$ are the head projection matrices.

Corresponding to our experiment, a head computation can be viewed as a fusion between the projected subspaces from each input modality.  
\newline
\textbf{Positional Encoding}.
%\subsubsection{Positional Encoding}
Every input token in the input sequence is converted to the learned embeddings first. Nonetheless, the self attention module does not provide the temporal information during the computation. Therefore, the learned embedding will add a residual positional encoding to enhance the temporal information in the every time step input. The positional encoding is computed by 
%${PE}_{(pos, 2i)}   = sin(pos/{10000}^{\frac{2iH}{d}})$ and ${PE}_{(pos, 2i+1)} = cos(pos/{10000}^{\frac{2iH}{d}})$.
:
\begin{align}
    & {PE}_{(pos, 2i)}   = sin(pos/{10000}^{\frac{2iH}{d}}) \\
    & {PE}_{(pos, 2i+1)} = cos(pos/{10000}^{\frac{2iH}{d}})
\end{align}
The residual positional encoding is then calculated by the input embedding multiplied by the positional encoding. The detailed math explanation of positional encoding could refer to \cite{transformer} for further explanation.
\newline
\textbf{Overall Architecture}
%\subsubsection{Overall Architecture}
The entire transformer architecture is composed of a multi-head attention block and a feed-forward block. In our experiment, the feed-forward block is a two-layered MLP. The entire process is described in Figure \ref{fig:transformer}.

%\begin{figure}
%  \includegraphics[width=0.45\textwidth, , height=0.3\textwidth]{figure/transformer.pdf}
%  \caption{The architecture of the cross-modal transformer encoder. The transformer encoder is composed of a stack of N identical layers as illustrated above. The transformer encoder takes 3 arguments as input, Value (V), Key (K) and Query (Q), and computes the self-attention value with multi-head attention layers and normalization layers. Inspired by the transformer architecture, we set $N=6$ and take V, K , and Q for different modalities. A head attention can be treated as a (learned) weight for the projected semantic subspace of a single modality. The multi-head attention allows the model to aggregate the rich and attentive information from different subspaces.} %% -W
%  \label{fig:transformer}
%\end{figure}
\fi

\iffalse
\section{Baseline Networks}\label{section: baseline}
We introduce two competitive single source baseline networks, \baseline{} \cite{S2VT}, OBJ2TEXT \cite{obj2text}, which is the backbone of most of the video captioning models and we build our multimodal baseline network by extending IMGD \cite{imgd}. %% -W

\subsection{Single Source Baseline Networks}
We investigate two baseline networks for single source VideoQG, including S2VT \cite{S2VT}, which comprehend video frames, and OBJ2TEXT \cite{obj2text}, which takes as object-level features. \footnote{Bounding boxes are not used for a fair comparison.} Both networks are implemented with two layers LSTM encoder and two layers LSTM decoder. 
%The LSTM encoder extracts the features from video frames and passes the features to the LSTM decoder. 
In the decoding stage, we apply Luong Attention \cite{LuongAttention} to capture contextual representation. The hyperparameters of the single source baseline models are listed in section \ref{section: details}.

\subsection{Multimodal Baseline Network: IMGD}
We apply Images for decoder initialisation (IMGD) \cite{imgd} as our multimodal baseline network. We pass different modal inputs through individual LSTM encoder to extract features for each modality. We incorporate the last hidden states of the two different LSTM encoders as the initial state of our LSTM decoder, following in \cite{imgd}. 
%The above fusion mechanism is followed by \cite{imgd}.
\fi


\if false \section{Related Wotk}
\label{sec: relatedwork}

\subsection{Visual Question Answering}
VQA can be split into two branches: image question answering and video question answering. Recently, several image question answering datasets have been built, including COCO-QA \cite{DBLP:conf/nips/RenKZ15}, VQA 1.0 \cite{VQA}, VQA 2.0 \cite{balanced_vqa_v2}, CLEVR \cite{DBLP:conf/cvpr/JohnsonHMFZG17}, and Visual7w \cite{DBLP:conf/cvpr/ZhuGBF16}. Similar to image QA, a number of Video QA datasets have been proposed. PororoQA \cite{DBLP:conf/ijcai/KimHCZ17} and MarioQA \cite{DBLP:conf/iccv/MunSJH17} are constructed from the unrealistic video sources. MovieQA \cite{DBLP:conf/cvpr/TapaswiZSTUF16} dataset is built upon language sources, while MovieFIB \cite{DBLP:conf/cvpr/MaharajBRCP17}, VideoQA \cite{xu2017video}, TGIFQA \cite{DBLP:conf/cvpr/JangSYKK17} are based on visual sources. As for the data collection strategy of TVQA \cite{tvqa} dataset, humans are required to focus on both the visual and language sources to label the dataset.

\subsection{Question Generation}
The question generation tasks can be categorized in terms of the input modality, which are the textual and visual features. Text-based question generation has attracted the natural language community in recent years due to the huge cost of human labeling. NQG
\cite{L2A} with the seq2seq based framework is able to generate a question given a text passage. There are also works about image-based question generation. 
Mostafazadeh et al. 
\cite{conf/acl/MostafazadehMDM16} aims to generate a natural and engaging question when shown an image. They proposed Gated Recurrent Neural Network and a retrieval based model which leverages the training labels to generate questions.  
Li et al. 
\cite{DBLP:conf/cvpr/LiDZCOWZ18} introduce question generation as a dual task of question answering. They exploit the inherent complementary relation between question answering and generation to generate questions and answers.
\fi
%


%tasks: QG, DQG
%rows:
%cols: BLEU4, ROUGE, CIDEr, SPICE, METEOR

%\def\methodc{Joint-QA Decoder}
\begin{table*}\label{table:div1}
    \centering
    \begin{tabular}{
    |lll|
    c|c|c|
    c|c|c|
    c|c|c|
    c|c|c|
    }%c|c|}%c|c|c|c|}
    \hline
    %& TVQA & \multicolumn{2}{c|}{BLEU-4} & 
    %\multicolumn{2}{c|}{ROUGE} &
    %\multicolumn{2}{c|}{CIDEr} &
    %\multicolumn{2}{c|}{METEOR} 
    %\multicolumn{2}{c|}{+100\%}
    %\\ \hline
    %& \localized & \unlocalized 
     %& \localized & \unlocalized
     %& \localized & \unlocalized
     %& \localized & \unlocalized
     & &
     & \multicolumn{3}{|c|}{Unigram}
     & \multicolumn{3}{|c|}{Bigram}
     & \multicolumn{3}{|c|}{Noun}
     & \multicolumn{3}{|c|}{Verb}
    \\
    &  &
    & 0.1\%
    & 1\%
    & 10\%
    & 0.1\%
    & 1\%
    & 10\%
    & 0.1\%
    & 1\%
    & 10\%
    & 0.1\%
    & 1\%
    & 10\%
    \\ \hline
    
    & \multirow{3}{*}{w/o subtitle} 
    & \baseline \cite{S2VT}
    %& 0.7226 & 0.9997 & 1.0000 
    %& 0.8785 & 1.0000 & 1.0000
    %& 0.6139 & 1.0000 & 1.0000
    %& 0.3906 & 0.9999 & 1.0000
    & 0.722 & 0.999 & 1.000 
    & 0.878 & 1.000 & 1.000
    & 0.613 & 1.000 & 1.000
    & 0.390 & 0.999 & 1.000
    \\
    %& \baselinea
    %& 0.1044 & 0.3849 & 0.0642 & 0.1533
    %\\
    & & \methodb %(V) 
    & 0.3941 & 0.9311 & 0.9991 
    & 0.5834 & 0.9137 & 1.0000
    & 0.4302 & 0.7750 & 0.9616
    & 0.3150 & 0.9146 & 0.9914
    \\
    %& \methodb (O)
    %& 0.1320 & 0.4136 & 0.1750 & 0.1803
    %\\
    & & \methodaa + \methodb
    & \textbf{0.3384} & \textbf{0.8798} & \textbf{0.9801} 
    & 0.4867 & 0.8114 & 0.9791
    & 0.4429 & 0.8898 & 1.0000
    & 0.4949 & 0.9955 & 1.0000
    \\
    \hline
    
    & \multirow{3}{*}{w/ subtitle} 
    & \multibaseline  \cite{imgd}
    & \textbf{0.3452} & 0.9995 & 1.0000 
    & 0.6805 & 1.0000 & 1.0000
    & 0.5764 & 1.0000 & 1.000
    & 0.3195 & 0.9993 &1.0000
    \\
    & & \methodb 
    & 0.4042 & \textbf{0.9590}& 1.0000 
    & 0.6630 & 0.9800 & 1.0000
    & 0.4429 & 0.8898 & 1.0000
    & 0.4949 & 0.9955 & 1.0000
    \\
    %& Multimodal \methoda + \methodb
    %& 0.1441 & 0.4217 & 0.2363 & 0.1898
    %\\
    & &  \methodaa + \methodb
    & 0.4395 & 0.9801 & 1.0000 
    & 0.6886 & 0.9929 & 1.0000
    & 0.4257 & 0.9534 &1.0000
    & 0.5295 & 0.9972 & 1.0000
    \\
    \hline
    & & GT (Oracle)
    & 0.2545 & 0.6631 & 0.8646
    & 0.1641 & 0.3876 & 0.6477
    & 0.3160 & 0.4923 & 0.7956
    & 0.1693 & 0.5702 & 0.8426
    \\
    \hline
    \end{tabular}
    \caption{Frequent Word Coverage for Unigram, Bigram, Noun and Verb. The lower the more diverse. 
    %Most frequent unigrams and bigrams coverage in the generated and ground truth questions. %As we aim to train the Video QA model with the generated questions, 
    %The questions is preferable to be diverse to enable the model to understand user generated questions. 
    %However, neural network based Video QG models tend to overestimate the frequent words especially it does not well understand the input features.
    Our model significantly surpasses the strong baseline model in the video-only scenario (First Block), while in the video+subtitle scenario, the frequent words coverage slightly increase. On the other hand, the baseline models has less frequent words coverage while having less scores in Table \ref{table:results}, revealing that the models copy from the subtitles source, which increases diversity but still obtaining low scores in Table \ref{table:results}.
    %We compare our proposed method with a competitive video captioning model based on a previous work. \cite{S2VT}.
    First block: Training with video only without subtitles. Second block: Training with both video and subtitles. Our proposed method significantly outperforms the strong baseline in both scenario. Last block: Human labeled ground truth questions as the oracle case.(cf. Section\ref{section:div})
    }
    \label{table:divbig}
\end{table*}


==> figure/diversity1.tex <==


%tasks: QG, DQG
%rows:
%cols: BLEU4, ROUGE, CIDEr, SPICE, METEOR

%\def\methodc{Joint-QA Decoder}
\begin{table*}\label{table:div1}
    \centering
    \begin{tabular}{
    |lll|
    c|c|c|
    c|c|c|
    }%c|c|}%c|c|c|c|}
    \hline
    %& TVQA & \multicolumn{2}{c|}{BLEU-4} & 
    %\multicolumn{2}{c|}{ROUGE} &
    %\multicolumn{2}{c|}{CIDEr} &
    %\multicolumn{2}{c|}{METEOR} 
    %\multicolumn{2}{c|}{+100\%}
    %\\ \hline
    %& \localized & \unlocalized 
     %& \localized & \unlocalized
     %& \localized & \unlocalized
     %& \localized & \unlocalized
     & &
     & \multicolumn{3}{|c|}{Unigram}
     & \multicolumn{3}{|c|}{Bigram}
    \\
    &  &
    & 0.1\%
    & 1\%
    & 10\%
    & 0.1\%
    & 1\%
    & 10\%
    \\ \hline
    
    & \multirow{3}{*}{w/o subtitle} 
    & \baseline \cite{S2VT}
    & 0.7226 & 0.9997 & 1.0000 
    & 0.8785 & 1.0000 & 1.0000
    \\
    %& \baselinea
    %& 0.1044 & 0.3849 & 0.0642 & 0.1533
    %\\
    & & \methodb %(V) 
    & 0.3941 & 0.9311 & 0.9991 
    & 0.5834 & 0.9137 & 1.0000
    \\
    %& \methodb (O)
    %& 0.1320 & 0.4136 & 0.1750 & 0.1803
    %\\
    & & \methodaa + \methodb
    & \textbf{0.3384} & \textbf{0.8798} & \textbf{0.9801} 
    & 0.4867 & 0.8114 & 0.9791
    \\
    \hline
    
    & \multirow{3}{*}{w/ subtitle} 
    & \multibaseline  \cite{imgd}
    & \textbf{0.3452} & 0.9995 & 1.0000 
    & 0.6805 & 1.0000 & 1.0000
    \\
    & & \methodb 
    & 0.4042 & \textbf{0.9590}& 1.0000 
    & 0.6630 & 0.9800 & 1.0000
    \\
    %& Multimodal \methoda + \methodb
    %& 0.1441 & 0.4217 & 0.2363 & 0.1898
    %\\
    & &  \methodaa + \methodb
    & 0.4395 & 0.9801 & 1.0000 
    & 0.6886 & 0.9929 & 1.0000
    \\
    \hline
    & & Ground Truth (Oracle)
    & 0.2545 & 0.6631 & 0.8646
    & 0.1641 & 0.3876 & 0.6477
    \\
    \hline
    \end{tabular}
    \caption{Frequent Word Coverage. The lower the more diverse. Most frequent unigrams and bigrams coverage in the generated and ground truth questions. %As we aim to train the Video QA model with the generated questions, 
    %The questions is preferable to be diverse to enable the model to understand user generated questions. 
    %However, neural network based Video QG models tend to overestimate the frequent words especially it does not well understand the input features.
    Our model significantly surpasses the strong baseline model in the video-only scenario (First Block), while in the video+subtitle scenario, the frequent words coverage slightly increase. On the other hand, the baseline models has less frequent words coverage while having less scores in Table \ref{table:results}, revealing that the models copy from the subtitles source, which increases diversity but still obtaining low scores in Table \ref{table:results}.
    %We compare our proposed method with a competitive video captioning model based on a previous work. \cite{S2VT}.
    First block: Training with video only without subtitles. Second block: Training with both video and subtitles. Our proposed method significantly outperforms the strong baseline in both scenario. (cf. Section\ref{section:div})
    }
    \label{table:div1}
\end{table*}


==> figure/diversity2.tex <==


%tasks: QG, DQG
%rows:
%cols: BLEU4, ROUGE, CIDEr, SPICE, METEOR

%\def\methodc{Joint-QA Decoder}
\begin{table*}\label{table:div2}
    \centering
    \begin{tabular}{
    |lll|
    c|c|c|
    c|c|c|
    }%c|c|}%c|c|c|c|}
    \hline
    %& TVQA & \multicolumn{2}{c|}{BLEU-4} & 
    %\multicolumn{2}{c|}{ROUGE} &
    %\multicolumn{2}{c|}{CIDEr} &
    %\multicolumn{2}{c|}{METEOR} 
    %\multicolumn{2}{c|}{+100\%}
    %\\ \hline
    %& \localized & \unlocalized 
     %& \localized & \unlocalized
     %& \localized & \unlocalized
     %& \localized & \unlocalized
     & &
     & \multicolumn{3}{|c|}{Noun}
     & \multicolumn{3}{|c|}{Verb}
    \\
    &  &
    & 0.1\%
    & 1\%
    & 10\%
    & 0.1\%
    & 1\%
    & 10\%
    \\ \hline
    
    & \multirow{3}{*}{w/o subtitle} 
    & \baseline \cite{S2VT}
    & 0.6139 & 1.0000 & 1.0000
    & 0.3906 & 0.9999 & 1.0000
    \\
    %& \baselinea
    %& 0.1044 & 0.3849 & 0.0642 & 0.1533
    %\\
    & & \methodb %(V) 
    & 0.3596 & 0.8295 & 0.9952
    & 0.4616 & 0.9662 & 1.0000
    \\
    %& \methodb (O)
    %& 0.1320 & 0.4136 & 0.1750 & 0.1803
    %\\
    & & \methodaa + \methodb
    & 0.4302 & 0.7750 & 0.9616
    & 0.3150 & 0.9146 & 0.9914
    \\
    \hline
    
    & \multirow{3}{*}{w/ subtitle} 
    & \multibaseline \cite{imgd}
    & 0.5764 & 1.0000 & 1.000
    & 0.3195 & 0.9993 &1.0000
    \\
    & & \methodb 
    & 0.4429 & 0.8898 & 1.0000
    & 0.4949 & 0.9955 & 1.0000
    \\
    %& Multimodal \methoda + \methodb
    %& 0.1441 & 0.4217 & 0.2363 & 0.1898
    %\\
    & &  \methodaa + \methodb
    & 0.4257 & 0.9534 &1.0000
    & 0.5295 & 0.9972 & 1.0000
    \\
    \hline
    & & Ground Truth (Oracle)
    & 0.3160 & 0.4923 & 0.7956
    & 0.1693 & 0.5702 & 0.8426
    \\
    \hline
    \end{tabular}
    \caption{\textbf{Frequent Nouns and Verbss Coverage} 
    % Should have more descriptions
    We tokenize the generated and ground truth questions with NLTK \cite{nltk}.
    }
    \label{table:div2}
\end{table*}

